2-dimensional unit vector flows

We study $2$-dimensional unit vector flows on graphs, that is, nowhere-zero flows that assign to each oriented edge a unit vector in $\mathbb R^{3}$. We give a new geometric characterization of $\mathbb S^{2}$-flows on cubic graphs. We also prove that the class of cubic graphs admitting an $\mathbb S^{2}$-flow is closed under a natural composition operation, which yields further constructions; in particular, blowing up a vertex into a triangle preserves the existence of an $\mathbb S^{2}$-flow. Our second contribution is algebraic: we extend the rank-based approach of [SIAM J. Discrete Math., 29 (2015), pp.~2166--2178] from $\mathbb S^{1}$-flows to $\mathbb S^{2}$-flows. More precisely, we show that if an $\mathbb S^{2}$-flow $\varphi$ satisfies $\operatorname{rank}(S_{\mathbb{Q}}(\varphi))\le 2$ and $S_{\mathbb{Q}}(\varphi)$ is odd-coordinate-free, then the graph admits a nowhere-zero $4$-flow.

==> deleted.tex <==
\hussein{The old proof!}

Consider a vector $v = (v_x, v_y, v_z) \in \SSS^2$, we define the \defin{root plane} of $v$, denoted by $\mathcal{P}_v$, as the plane with normal vector $v$ and contains the point $\frac{-1}{\sqrt{2}}(v_x, v_y, v_z)$. Precisely, $\mathcal{P}_v$ satisfies the following equation.
\begin{equation}
    v_x\cdot x + v_y \cdot y + v_z \cdot z + \frac{1}{\sqrt{2}}v_x^2 + \frac{1}{\sqrt{2}}v_y^2 + \frac{1}{\sqrt{2}}v_z^2 = 0
\end{equation}

We define the \defin{root circle} of a vector $v \in \SSS^2$  as the intersection of $\mathcal{P}_v$ and $\SSS^2$.

\begin{obs}
    Let $u, w$ be any two diametrically opposite points on $C_v$ for some $v \in \SSS^2$, then $u + v + w = \overrightarrow{0}$. The angle between any of $u, v, w$ is $2\pi/3$. 
\end{obs}

\begin{thm}
Let $G$ be a cubic graph. If $G$ admits an $\SSS^2$-flow, then the graph obtained by blowing up any vertex in $V(G)$ into a triangle also admits an $\SSS^2$-flow.
\end{thm}
\begin{proof}
Take a vertex $x \in V(G)$, let $e_1, e_2, e_3 \in E(G)$ be the incident arcs to $x$ oriented away from $x$. Let $f$ be an $\SSS^2$-flow on $E(G)$, such that $f(e_1) = a$, $f(e_2) = b$, and $f(e_3) = c$. Since $f$ is a flow, we have $a + b + c = 0$. Now, replace $x$ by the triangle $T = \{u, v, w\}$ and orient the edges of $T$ from $u$ to $v$, from $v$ to $w$, and from $w$ to $u$. Let $u$, $v$, and $w$ each inherit the arc $e_1$, $e_2$, and $e_3$ respectively. Now define a new $\SSS^2$-flow $g$, $g$ equals to $f$ on every arc, and in the remaining of the proof we will define $g$ on $\overrightarrow{uv}, \overrightarrow{vw}, \overrightarrow{wu}$. Let $i$, $j$, and $k$ denotes the variables $g(\overrightarrow{uv}), g(\overrightarrow{vw}), g(\overrightarrow{wu})$. We want show that $i, j, k$ exists and they satisfy the following constraints. 
\begin{equation}\label{constraints}
\begin{cases}
    a + i - k = 0\\
    b - i + j = 0\\
    c - j + k = 0
\end{cases}    
\end{equation}
Let $C_a$, $C_b$, and $C_c$ be the root circles of $a, b$ and $c$ respectively. We also refer to $-C_a, -C_b,$ and $-C_c$ as the root circle of $-a, -b$, $-c$ instead of $C_{-a}, C_{-b}$, and $C_{-c}$ as they are symmetric with respect to the origin.
From \cref{constraints}, we can conclude the following. 
\begin{enumerate}
    \item $\{i, -k\} \subseteq C_a$
    \item $\{-i, j\} \subseteq C_b$
    \item $\{-j, k\} \subseteq C_c$
\end{enumerate}
We can rearrange these relations as,
\begin{enumerate}
    \item $i \in C_a \cap -C_b$
    \item $j \in C_b \cap -C_c$
    \item $k \in C_c \cap -C_a$
\end{enumerate}
Observe that $-C_a, -C_b, -C_c$ are the rotation of $C_a, C_b, C_c$ by $\pi$.

\hussein{now, I want to say that these circles intersects without solving any equation. Probably I can use the intermediate value theorem on the rotation taking $C_b$ to $C_c$.}
\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.7]{figs/Solution for triangle s2 flow.png}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

\end{proof}

Let $(D,f)$ be a vector $\SSS^{2}$–flow on a graph $G$.  Its set of flow
values is
\[
  \{f(e)\mid e\in E(G)\}\;=\;\{\pm\alpha_{1},\pm\alpha_{2},\dots,\pm\alpha_{b}\},
\]
where $\{\alpha_{1},\alpha_{2},\dots,\alpha_{b}\}\subseteq \SSS^{2}$ consists of
$b$ pairwise linearly independent vectors.

Without loss of generality we may further assume that
\[
  \{f(e)\mid e\in E(G)\} \;=\; \{\alpha_{1},\alpha_{2},\dots,\alpha_{k}\},
\]
because whenever an edge $e$ satisfies $f(e)=-\alpha_{i}$ we simply reverse the
orientation of $e$ and replace its flow value by $-\!f(e)=\alpha_{i}$.
\begin{defn}
For a vertex $v$, define the \defin{balanced vector} $\boldsymbol{\epsilon}(v) \in \mathbb{Z}^b$ as:
\[
\boldsymbol{\epsilon}(v) = \left( \epsilon_1(v), \dots, \epsilon_b(v) \right),
\]
where $\epsilon_i(v) = |E^+(v) \cap E_i| - |E^-(v) \cap E_i|$, and $E_i$ is the set of edges with flow value $\boldsymbol{\alpha}_i$.
\end{defn}

\begin{defn}
Let  $\boldsymbol{f}$ be an $\SSS^2$-flow of $G$ with an orientation $D$.
The \defin{rank} of $(D, \boldsymbol{f})$ is the dimension of the subspace $S(\boldsymbol{f}) \subset \mathbb{R}^b$ spanned by all balanced vectors $\boldsymbol{\epsilon}(v)$.
\end{defn}


\begin{thm}
If $G$ admits an $\SSS^2$-flow with rank $\leq 3$, then $G$ admits a nowhere-zero $4$-flow. This result is sharp.
\end{thm}

\begin{proof}
Let $(D, \boldsymbol{f})$ be an $\SSS^2$-flow with rank $\leq 3$. The balanced vectors $\{\boldsymbol{\epsilon}(v)\}$ span a subspace $S(\boldsymbol{f}) \subset \mathbb{R}^3$. Choose a basis $\{\boldsymbol{\eta}_1, \boldsymbol{\eta}_2, \boldsymbol{\eta}_3\}$ for $S(\boldsymbol{f})$.

For each edge $e$, write $\boldsymbol{f}(e) = c_1(e) \boldsymbol{\eta}_1 + c_2(e) \boldsymbol{\eta}_2 + c_3(e) \boldsymbol{\eta}_3$, where $c_i(e) \in \mathbb{Q}$ \hussein{we computed the rank over $\{\epsilon(v)\}$, so for any $v$, $\epsilon(v) = c_1\eta_1 + c_2\eta_2 + c_3\eta_3$, how we moved from this to the edge case?}. Scale the flow to clear denominators, obtaining integer coefficients $\tilde{c}_i(e) \in \{\pm 1, \pm 2, \pm 3\}$.
\hussein{Why the coefficient in $\mathbb{Q}$?, we can change the basis so that works for a particular edge but not sure if it will work for all $e \in E$.}

 Define $f(e) = \tilde{c}_1(e) + \tilde{c}_2(e) + \tilde{c}_3(e)$. By linear independence of $\{\boldsymbol{\eta}_i\}$, flow conservation is preserved:
\[
\sum_{e \in E^+(v)} f(e) - \sum_{e \in E^-(v)} f(e) = 0 \quad \forall v \in V(G).
\]
Thus, $(D, f)$ is a nowhere-zero integer $4$-flow.

[Possible Candidate: A planar graph dual to a 3D unit distance graph with chromatic number 5 (e.g., a 4-regular graph requiring rank $\geq 4$) admits an $\SSS^2$-flow but no integer $4$-flow.]
\end{proof}

\begin{thm}
If $G$ admits a vector $\SSS^2$-flow with rank $\leq 3$, then $G$ is either Eulerian (admitting a $2$-flow) or has a circular $\left(3 + \frac{1}{p}\right)$-flow for some $p \geq 1$.
\end{thm}

\begin{proof}
1. \textbf{Case 1: Eulerian Graphs:} If all vertices have even degrees, orient edges consistently along an Eulerian circuit. Assign $f(e) = \pm 1$ alternately, yielding a nowhere-zero $2$-flow.

2. \textbf{Case 2: Non-Eulerian Graphs:} 
   - By Jaeger’s theorem, $G$ has a modulo $(3p + 1)$-orientation for some $p \geq 1$.
   - Assign flow values $\pm 1, \dots, \pm 3p$ to edges such that:
     \[
     \sum_{e \in E^+(v)} f(e) - \sum_{e \in E^-(v)} f(e) \equiv 0 \pmod{3p + 1}.
     \]
   - The rank condition ensures this system has a solution, giving a circular $\left(3 + \frac{1}{p}\right)$-flow.
\end{proof}

\begin{thm}
Let $G$ be a graph where $V_4$ (degree-4 vertices) induces a connected subgraph and $G - V_4$ is acyclic. Then $G$ admits a nowhere-zero integer $4$-flow if and only if it admits a vector $\SSS^2$-flow.
\end{thm}

\begin{proof}
1. \textbf{Forward Direction ($\Rightarrow$):} An integer $4$-flow directly induces an $\SSS^2$-flow by mapping flow values to orthogonal unit vectors (e.g., $1 \mapsto \mathbf{e}_x, 2 \mapsto \mathbf{e}_y$, etc.).

2. \textbf{Reverse Direction ($\Leftarrow$):} 
     - $G - V_4$ is acyclic, so all cycles are in $G[V_4]$.
     - $G[V_4]$ is connected, allowing flow propagation.
     - For each $v \in V_4$, the $\SSS^2$-flow equation $\boldsymbol{\alpha}_1 + \boldsymbol{\alpha}_2 + \boldsymbol{\alpha}_3 + \boldsymbol{\alpha}_4 = \mathbf{0}$ implies linear dependence. Assign integers $\pm 1, \pm 2, \pm 3$ to edges via Gaussian elimination on the balanced vectors.
Remove a degree-4 vertex $v$, split its edges into pairs $(e_1, e_2)$ and $(e_3, e_4)$, and preserve flow consistency. Reconstruct the integer flow inductively.

 If $V_4$ is disconnected, two disjoint copies of $K_5$ (non-planar) admit $\SSS^2$-flows but no integer $4$-flows.
\end{proof}
\end{enumerate}
\begin{figure}[H]
\centering
\subfloat[\centering ]{{\includegraphics[scale=0.50]{figs/dual_C4_car_k2.pdf}}}
\qquad
\subfloat[\centering Draw of $S^2$-immersion]{{\includegraphics[scale=0.50]{figs/dual_C4_car_k2.pdf} }}%
\caption{sdfsdfdsfsf}
\label{fig:sjgfsdkfsdfhjsk}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In \cite{VecAndInt}, they prove the following, 
\begin{lem}
    Suppose that $G$ admits a vector $\SSS^1$-flow $f$ with rank at most one, and let $D$ be an orientation of $E(G)$, and let $H$ be the core of $G$. Then, 
    \begin{enumerate}
        \item $H$ is a $k^*$-regular bipartite graph with vertex bi-partition $(A, B)$, where 
        $$A = \{v\in V(H): \epsilon(v) = \epsilon\}, \quad B = \{v\in V(H): \epsilon(v) = -\epsilon \} $$
        \item $H$ admits a vector $\SSS^1$-flow, say $(D_h, f_h)$, and $S(f_h) = S(f)$;
        \item $H$ has a $K^*$-orientation and therefore $G$ a modulo $k^*$-orientation;
        \item for each $i=1,2,..., b$, $E_i(H)$ can be decomposed into $|\epsilon_i|$ perfect matching of $H$, denoted by $M_1, ..., M_{|\epsilon_i|}$.
    \end{enumerate}
\end{lem}
From this lemma, we get the following theorem. 
\begin{thm}
    If a graph $G$ admits a vector $\SSS^1$-flow with rank at most one, then either $G$ is Eulerian and thus admits a nowhere-zero integer $2$-flow, or $G$ admits a circular $(2 + \frac{1}{p})$-flow for some integer $p$ with $k^* = 2p + 1$ and $p \geq 1$.
\end{thm}
\hussein{In the proof of this theorem, I still do not see where $\SSS^1$-flow is used, I think that's true for any subspace with dimension (or rank) at most one. I think also part $(b)$ of the lemma above follows from part $(a)$ and \cref{cubic} (assuming that the process in Figure 1. does not break bipartiteness!).}

% A \defin{direction} of $ C $ \hussein{What is $C$, a cycle?  or any subgraph} is an ordered pair $ (X, Y) $ of disjoint subsets of $ E(C) $ whose union is $ E(C) $, such that every $ e \in X $ and $ f \in Y $ have opposite orientations with respect to $ C $ \hussein{do we use this anywhere? I do not think so}.
% We call the edges in $ X $ ``forward edges'' and the edges in $ Y $ ``backward edges".  

We now follow the framework of Jaeger in \cite{Jaeger} by defining a restricted class of flows. Let $ \Bcal \subseteq \Acal $ be a subset of an abelian group $ \Acal $, and assume that $ -\Bcal = \Bcal $. (That is, the inverse of each element in $ \Bcal $ is also in $ \Bcal $.)
If $ \varphi \colon E(\vec{G}) \to \Acal $ is a $\Acal$-flow such that $\varphi(E(\vec{G})) \subseteq \Bcal $, then we say that $ \varphi $ is a \defin{$\Bcal $-flow}.
%We say that a flow  $ \varphi $ is \defin{nowhere-zero} if it is an $ (\Acal \sm \{0\}) $-flow.

If $\varphi$ is a $ \Bcal $-flow on $ \vec{G} $, and we reverse the orientation of some edge $e \in E(\vec{G})$, then replacing $\varphi(e)$ by its inverse ensures that $ \varphi $ remains a $ \Bcal $-flow \hussein{not sure if this is necessary!}.
Thus, for an undirected graph $ G $, we say that $G$ has a $ \Bcal $-flow if some (and hence every) orientation of $G$ admits such a flow.

% \hussein{this is too long! The old thing.} 
% Let $ r \ge 2 $ be a real number and $d$ a positive integer. An $(r, d)$-flow on $G$ is a function $\varphi \colon E(G) \to \mathbb{R}^d$ such that, for every edge $e \in E(G)$, the Euclidean norm of $\varphi(e)$ lies in the interval $ [1, r - 1]$, and for every vertex $ v \in V(G) $, the sum of the flow vectors on the incoming and outgoing edges is the zero vector in $ \mathbb{R}^d $.


% In this paper, we focus on $ (2, d) $-NZFs.

% More precisely, we define the following notation:

% Let $ (V, \|\,\cdot\,\|) $ be a vector space over a field $ \F $, equipped with a norm $ \|\,\cdot\,\|$.  
% A \defin{unit vector $ V $-flow with respect to $ \|\,\cdot\,\| $} on a graph $ G $ is a flow whose values are unit vectors in $ V $, i.e., the elements of the set $ \{ v \in V \mid \|v\| = 1 \} $.
% For simplicity, if $ \dim_{\F} V = n+1 $, we refer to such a flow as an $ \SSS^n $-flow with respect to the norm $ \|\,\cdot\,\| $ over $ \F $.


%\textit{The old proof.}
%Suppose an edge $e$ collapses to a single point on $\SSS^2$. Then $e$ must lie along a great circle in $\SSS^2$. Let $e_1$ and $e_2$ be the two edges incident to $e$. Without loss of generality, assume one of these incident edges has endpoints whose images in $\SSS^2$ are distinct. But that immediately contradicts the angle condition. Therefore, the endpoints of every edge must map to two distinct points on $\SSS^2$; in particular, one of those points can be taken to be the north pole and the other the south pole.
%We then apply Pat's lemma to obtain a one-point $ \mathbb{S}^2 $-immersion.

%A stronger results holds for a 3-edge-colourable cubic graph $G$, they show $f_2(G) \le 1 + \sqrt{2}$ ; see \cite[Proposition 3.2]{NZF}. 

Unit vector flows are studied mostly in \cite{VecAndInt,thom2}. \citet{VecAndInt} answer a specific case of \cref{problem1}. They show that if a graph $G$ admits an $\SSS^1$-flow with rank at most two, then $G$ admits a $3$-flow \cite{VecAndInt}; Note that the rank of an $\SSS^1$-flow is defined similarly as above. 
A precise characterisation for graphs admitting $\SSS^1$-flows is given in \cite[Proposition 1]{thom2}. Furthermore, \cite{thom2} studies the relation between unit vector flows and the edge connectivity of a graph.

For an abelian group $\Acal$ and a subset $\calF \subseteq \Acal$,  \citet{thom2} defines $\lambda(\calF, \Acal)$ as the smallest natural number such that a $\lambda(\calF, \Acal)$-edge-connected graph has an $\calF$-flow. For a one dimensional unit sphere, the following inequality holds $4 \leq \lambda(\SSS^1, \mathbb{R}^2) \leq \lambda(R_3, \mathbb{C}) \leq 6$ where $R_3$ is the set of complex numbers $z$ satisfying $z^3 = 1$, see \cite{thom2, LOVASZ2013587}.
For a two dimensional unit sphere, we have $\lambda(\SSS^2, \mathbb{R}^3) \leq \lambda(T, \mathbb{R}^3) = 4$, where $$T = \{(1, 1, 0), (0, 1, 1), (1, 0, 1), (1, -1, 0), (0, 1, -1), (1, 0, -1)\} \subseteq \mathbb{R}^3,$$ 
see \cite{thom2}. 
Note that \cref{Bobby_conj} is equivalent to showing $\lambda(\SSS^2, \mathbb{R}^3) = 2$.

For higher-dimensional unit spheres, a covering result of \citet{ber} implies that every $2$-edge-connected graph has an $\SSS^6$-flow. Another conjecture of \citet{fulkerson1971blocking} that involves covering graphs if true, would imply that every $2$-edge-connected graph has an $\SSS^5$-flow. Another covering conjecture of \citet{celmins1986cubic} and \citet{preissmann1981colorations} implies that every $2$-edge-connected graph has an $\SSS^4$-flow. On the other direction, vector flows have been used to derive covering results. Using vector flows, \citet{thom2} shows that for an odd natural number $k \geq 3$, every $(3k - 1)$-edge connected graph has a collection of $k$ even subgraphs such that every edge in $G$ is in precisely $k - 1$ of them.


authors. For instance, \citet{NZF} study the upper bound on $f_2(G)$ for every bridgeless graph. 
They show if $G$ is a bridgeless graph, then $f_2(G) \le 1 + \sqrt{5} $; see \cite[Proposition 2.4]{NZF}. 


\hussein{this might change!}


\bobby{It doesn't have a right flow and coherence.}
In the remaining of this paper, \cref{prelim} is dedicated to preliminaries we need to prove our main theorems \cref{thm:S2} and \cref{rank_odd_cor}. In \cref{proof_of_geometric_theorem} we prove \cref{thm:S2}. Then, we illustrate the use of \cref{thm:S2} in \cref{examples}. Finally, we prove \cref{rank_odd_cor} in \cref{proof_of_algebraic_thm}.

